Denmark's Participation in the Search Engine TREC COVID-19 Challenge: Lessons Learned about Searching for Precise Biomedical Scientific Information on COVID-19

This report describes the participation of two Danish universities, University of Copenhagen and Aalborg University, in the international search engine competition on COVID-19 (the 2020 TREC-COVID Challenge) organised by the U.S. National Institute of Standards and Technology (NIST) and its Text Retrieval Conference (TREC) division. The aim of the competition was to find the best search engine strategy for retrieving precise biomedical scientific information on COVID-19 from the largest, at that point in time, dataset of curated scientific literature on COVID-19 -- the COVID-19 Open Research Dataset (CORD-19). CORD-19 was the result of a call to action to the tech community by the U.S. White House in March 2020, and was shortly thereafter posted on Kaggle as an AI competition by the Allen Institute for AI, the Chan Zuckerberg Initiative, Georgetown University's Center for Security and Emerging Technology, Microsoft, and the National Library of Medicine at the US National Institutes of Health. CORD-19 contained over 200,000 scholarly articles (of which more than 100,000 were with full text) about COVID-19, SARS-CoV-2, and related coronaviruses, gathered from curated biomedical sources. The TREC-COVID challenge asked for the best way to (a) retrieve accurate and precise scientific information, in response to some queries formulated by biomedical experts, and (b) rank this information decreasingly by its relevance to the query. In this document, we describe the TREC-COVID competition setup, our participation to it, and our resulting reflections and lessons learned about the state-of-art technology when faced with the acute task of retrieving precise scientific information from a rapidly growing corpus of literature, in response to highly specialised queries, in the middle of a pandemic.

==> acronyms.tex <==
\acrodef{3G}[3G]{Third Generation Mobile System}
\acrodef{5S}[5S]{Streams, Structures, Spaces, Scenarios, Societies}
\acrodef{AAAI}[AAAI]{Association for the Advancement of Artificial Intelligence}
\acrodef{AAL}[AAL]{Annotation Abstraction Layer}
\acrodef{AAM}[AAM]{Automatic Annotation Manager}
\acrodef{ACLIA}[ACLIA]{Advanced Cross-Lingual Information Access}
\acrodef{ACM}[ACM]{Association for Computing Machinery}
\acrodef{ADSL}[ADSL]{Asymmetric Digital Subscriber Line}
\acrodef{ADUI}[ADUI]{ADministrator User Interface}
\acrodef{AIP}[AIP]{Archival Information Package}
\acrodef{AJAX}[AJAX]{Asynchronous JavaScript Technology and \acs{XML}}
\acrodef{ALU}[ALU]{Aritmetic-Logic Unit}
\acrodef{AMUSID}[AMUSID]{Adaptive MUSeological IDentity-service}
\acrodef{ANOVA}[ANOVA]{ANalysis Of VAriance}
\acrodef{ANSI}[ANSI]{American National Standards Institute}
\acrodef{AP}[AP]{Average Precision}
\acrodef{APC}[APC]{AP Correlation}
\acrodef{API}[API]{Application Program Interface}
\acrodef{AR}[AR]{Address Register}
\acrodef{AS}[AS]{Annotation Service}
\acrodef{ASAP}[ASAP]{Adaptable Software Architecture Performance}
\acrodef{ASI}[ASI]{Annotation Service Integrator}
\acrodef{ASL}[ASL]{Achieved Significance Level}
\acrodef{ASM}[ASM]{Annotation Storing Manager}
\acrodef{ASR}[ASR]{Automatic Speech Recognition}
\acrodef{ASUI}[ASUI]{ASsessor User Interface}
\acrodef{ATIM}[ATIM]{Annotation Textual Indexing Manager}
\acrodef{AUC}[AUC]{Area Under the ROC Curve}
\acrodef{AUI}[AUI]{Administrative User Interface}
\acrodef{AWARE}[AWARE]{Assessor-driven Weighted Averages for Retrieval Evaluation}
\acrodef{BANKS-I}[BANKS-I]{Browsing ANd Keyword Searching I}
\acrodef{BANKS-II}[BANKS-II]{Browsing ANd Keyword Searching II}
\acrodef{bpref}[bpref]{Binary Preference}
\acrodef{BNF}[BNF]{Backus and Naur Form}
\acrodef{BRICKS}[BRICKS]{Building Resources for Integrated Cultural Knowledge Services}
\acrodef{CAM}[CAM]{Convex Aggregating Measure}
\acrodef{CAN}[CAN]{Content Addressable Netword}
\acrodef{CAS}[CAS]{Content-And-Structure}
\acrodef{CBSD}[CBSD]{Component-Based Software Developlement}
\acrodef{CBSE}[CBSE]{Component-Based Software Engineering}
\acrodef{CB-SPE}[CB-SPE]{Component-Based \acs{SPE}}
\acrodef{CD}[CD]{Collaboration Diagram}
\acrodef{CD}[CD]{Compact Disk}
\acrodef{CENL}[CENL]{Conference of European National Librarians}
\acrodef{CIDOC CRM}[CIDOC CRM]{CIDOC Conceptual Reference Model}
\acrodef{CIR}[CIR]{Current Instruction Register}
\acrodef{CIRCO}[CIRCO]{Coordinated Information Retrieval Components Orchestration}
\acrodef{CG}[CG]{Cumulated Gain}
\acrodef{CL}[CL]{Curriculum Learning}
\acrodef{CLEF1}[CLEF]{Cross-Language Evaluation Forum}
\acrodef{CLEF}[CLEF]{Conference and Labs of the Evaluation Forum}
\acrodef{CLIR}[CLIR]{Cross Language Information Retrieval}
\acrodef{CM}[CM]{Continuation Methods}
\acrodef{CMS}[CMS]{Content Management System}
\acrodef{CMT}[CMT]{Campaign Management Tool}
\acrodef{CNR}[CNR]{Italian National Council of Research}
\acrodef{CO}[CO]{Content-Only}
\acrodef{COD}[COD]{Code On Demand}
\acrodef{CODATA}[CODATA]{Committee on Data for Science and Technology}
\acrodef{COLLATE}[COLLATE]{Collaboratory for Annotation Indexing and Retrieval of Digitized Historical Archive Material}
\acrodef{CP}[CP]{Characteristic Pattern}
\acrodef{CPE}[CPE]{Control Processor Element}
\acrodef{CPU}[CPU]{Central Processing Unit}
\acrodef{CQL}[CQL]{Contextual Query Language}
\acrodef{CRP}[CRP]{Cumulated Relative Position}
\acrodef{CRUD}[CRUD]{Create--Read--Update--Delete}
\acrodef{CS}[CS]{Characteristic Structure}
\acrodef{CSM}[CSM]{Campaign Storing Manager}
\acrodef{CSS}[CSS]{Cascading Style Sheets}
\acrodef{CU}[CU]{Control Unit}
\acrodef{CUI}[CUI]{Client User Interface}
\acrodef{CV}[CV]{Cross-Validation}
\acrodef{DAFFODIL}[DAFFODIL]{Distributed Agents for User-Friendly Access of Digital Libraries}
\acrodef{DAO}[DAO]{Data Access Object}
\acrodef{DARE}[DARE]{Drawing Adequate REpresentations}
\acrodef{DARPA}[DARPA]{Defense Advanced Research Projects Agency}
\acrodef{DAS}[DAS]{Distributed Annotation System}
\acrodef{DB}[DB]{DataBase}
\acrodef{DBMS}[DBMS]{DataBase Management System}
\acrodef{DC}[DC]{Dublin Core}
\acrodef{DCG}[DCG]{Discounted Cumulated Gain}
\acrodef{DCMI}[DCMI]{Dublin Core Metadata Initiative}
\acrodef{DCV}[DCV]{Document Cut--off Value}
\acrodef{DD}[DD]{Deployment Diagram}
\acrodef{DDC}[DDC]{Dewey Decimal Classification}
\acrodef{DDS}[DDS]{Direct Data Structure}
\acrodef{DF}[DF]{Degrees of Freedom}
\acrodef{DFI}[DFI]{Divergence From Independence}
\acrodef{DFR}[DFR]{Divergence From Randomness}
\acrodef{DHT}[DHT]{Distributed Hash Table}
\acrodef{DI}[DI]{Digital Image}
\acrodef{DIKW}[DIKW]{Data, Information, Knowledge, Wisdom}
\acrodef{DIL}[DIL]{\acs{DIRECT} Integration Layer}
\acrodef{DiLAS}[DiLAS]{Digital Library Annotation Service}
\acrodef{DIRECT}[DIRECT]{Distributed Information Retrieval Evaluation Campaign Tool}
\acrodef{DKMS}[DKMS]{Data and Knowledge Management System}
\acrodef{DL}[DL]{Digital Library}
\acrodefplural{DL}[DL]{Digital Libraries}
\acrodef{DLMS}[DLMS]{Digital Library Management System}
\acrodef{DLOG}[DL]{Description Logics}
\acrodef{DLS}[DLS]{Digital Library System}
\acrodef{DLSS}[DLSS]{Digital Library Service System}
\acrodef{DM}[DM]{Data Mining}
\acrodef{DO}[DO]{Digital Object}
\acrodef{DOI}[DOI]{Digital Object Identifier}
\acrodef{DOM}[DOM]{Document Object Model}
\acrodef{DoMDL}[DoMDL]{Document Model for Digital Libraries}
\acrodef{DP}[DP]{Discriminative Power}
\acrodef{DPBF}[DPBF]{Dynamic Programming Best-First}
\acrodef{DR}[DR]{Data Register}
\acrodef{DRIVER}[DRIVER]{Digital Repository Infrastructure Vision for European Research}
\acrodef{DTD}[DTD]{Document Type Definition}
\acrodef{DVD}[DVD]{Digital Versatile Disk}
\acrodef{EAC-CPF}[EAC-CPF]{Encoded Archival Context for Corporate Bodies, Persons, and Families}
\acrodef{EAD}[EAD]{Encoded Archival Description}
\acrodef{EAN}[EAN]{International Article Number}
\acrodef{E-A-T}[E-A-T]{Expertise, Authoritativeness, and Trustworthiness}
\acrodef{ECD}[ECD]{Enhanced Contenty Delivery}
\acrodef{ECDL}[ECDL]{European Conference on Research and Advanced Technology for Digital Libraries}
\acrodef{EDM}[EDM]{Europeana Data Model}
\acrodef{EG}[EG]{Execution Graph}
\acrodef{ELDA}[ELDA]{Evaluation and Language resources Distribution Agency}
\acrodef{ELRA}[ELRA]{European Language Resources Association}
\acrodef{EM}[EM]{Expectation Maximization}
\acrodef{EMMA}[EMMA]{Extensible MultiModal Annotation}
\acrodef{EPROM}[EPROM]{Erasable Programmable \acs{ROM}}
\acrodef{EQNM}[EQNM]{Extended Queueing Network Model}
\acrodef{ER}[ER]{Entity--Relationship}
\acrodef{ERR}[ERR]{Expected Reciprocal Rank}
\acrodef{ETL}[ETL]{Extract-Transform-Load}
\acrodef{FAST}[FAST]{Flexible Annotation Service Tool}
\acrodef{FIFO}[FIFO]{First-In / First-Out}
\acrodef{FIRE}[FIRE]{Forum for Information Retrieval Evaluation}
\acrodef{FN}[FN]{False Negative}
\acrodef{FNR}[FNR]{False Negative Rate}
\acrodef{FOAF}[FOAF]{Friend of a Friend}
\acrodef{FORESEE}[FORESEE]{FOod REcommentation sErvER}
\acrodef{FP}[FP]{False Positive}
\acrodef{FPR}[FPR]{False Positive Rate}
\acrodef{GIF}[GIF]{Graphics Interchange Format}
\acrodef{GIR}[GIR]{Geografic Information Retrieval}
\acrodef{GAP}[GAP]{Graded Average Precision}
\acrodef{GLM}[GLM]{General Linear Model}
\acrodef{GLMM}[GLMM]{General Linear Mixed Model}
\acrodef{GMAP}[GMAP]{Geometric Mean Average Precision}
\acrodef{GoP}[GoP]{Grid of Points}
\acrodef{GPRS}[GPRS]{General Packet Radio Service}
\acrodef{gP}[gP]{Generalized Precision}
\acrodef{gR}[gR]{Generalized Recall}
\acrodef{gRBP}[gRBP]{Graded Rank-Biased Precision}
\acrodef{GTIN}[GTIN]{Global Trade Item Number}
\acrodef{GUI}[GUI]{Graphical User Interface}
\acrodef{GW}[GW]{Gateway}
\acrodef{HCI}[HCI]{Human Computer Interaction}
\acrodef{HDS}[HDS]{Hybrid Data Structure}
\acrodef{HIR}[HIR]{Hypertext Information Retrieval}
\acrodef{HIT}[HIT]{Human Intelligent Task}
\acrodef{HITS}[HITS]{Hyperlink-Induced Topic Search}
\acrodef{HTML}[HTML]{HyperText Markup Language}
\acrodef{HTTP}[HTTP]{HyperText Transfer Protocol}
\acrodef{HSD}[HSD]{Honestly Significant Difference}
\acrodef{ICA}[ICA]{International Council on Archives}
\acrodef{ICSU}[ICSU]{International Council for Science}
\acrodef{IDF}[IDF]{Inverse Document Frequency}
\acrodef{IDS}[IDS]{Inverse Data Structure}
\acrodef{IEEE}[IEEE]{Institute of Electrical and Electronics Engineers}
\acrodef{IEI}[IEI]{Istituto della Enciclopedia Italiana fondata da Giovanni Treccani}
\acrodef{IETF}[IETF]{Internet Engineering Task Force}
\acrodef{IMS}[IMS]{Information Management System}
\acrodef{IMSPD}[IMS]{Information Management Systems Research Group}
\acrodef{indAP}[indAP]{Induced Average Precision}
\acrodef{infAP}[infAP]{Inferred Average Precision}
\acrodef{INEX}[INEX]{INitiative for the Evaluation of \acs{XML} Retrieval}
\acrodef{INS-M}[INS-M]{Inverse Set Data Model}
\acrodef{INTR}[INTR]{Interrupt Register}
\acrodef{IP}[IP]{Internet Protocol}
\acrodef{IPSA}[IPSA]{Imaginum Patavinae Scientiae Archivum}
\acrodef{IR}[IR]{Information Retrieval}
\acrodef{IRON}[IRON]{Information Retrieval ON}
\acrodef{IRON2}[IRON$^2$]{Information Retrieval On aNNotations}
\acrodef{IRON-SAT}[IRON-SAT]{\acs{IRON} - Statistical Analysis Tool}
\acrodef{IRS}[IRS]{Information Retrieval System}
\acrodef{ISAD(G)}[ISAD(G)]{International Standard for Archival Description (General)}
\acrodef{ISBN}[ISBN]{International Standard Book Number}
\acrodef{ISIS}[ISIS]{Interactive SImilarity Search}
\acrodef{ISJ}[ISJ]{Interactive Searching and Judging}
\acrodef{ISO}[ISO]{International Organization for Standardization}
\acrodef{ITU}[ITU]{International Telecommunication Union }
\acrodef{ITU-T}[ITU-T]{Telecommunication Standardization Sector of \acs{ITU}}
\acrodef{IV}[IV]{Information Visualization}
\acrodef{JAN}[JAN]{Japanese Article Number}
\acrodef{JDBC}[JDBC]{Java DataBase Connectivity}
\acrodef{JMB}[JMB]{Java--Matlab Bridge}
\acrodef{JPEG}[JPEG]{Joint Photographic Experts Group}
\acrodef{JSON}[JSON]{JavaScript Object Notation}
\acrodef{JSP}[JSP]{Java Server Pages}
\acrodef{JTE}[JTE]{Java-Treceval Engine}
\acrodef{KDE}[KDE]{Kernel Density Estimation}
\acrodef{KLD}[KLD]{Kullback-Leibler Divergence}
\acrodef{KLAPER}[KLAPER]{Kernel LAnguage for PErformance and Reliability analysis}
\acrodef{LAM}[LAM]{Libraries, Archives, and Museums}
\acrodef{LAM2}[LAM]{Logistic Average Misclassification}
\acrodef{LAN}[LAN]{Local Area Network}
\acrodef{LD}[LD]{Linked Data}
\acrodef{LEAF}[LEAF]{Linking and Exploring Authority Files}
\acrodef{LIDO}[LIDO]{Lightweight Information Describing Objects}
\acrodef{LIFO}[LIFO]{Last-In / First-Out}
\acrodef{LM}[LM]{Language Model}
\acrodef{LMT}[LMT]{Log Management Tool}
\acrodef{LOD}[LOD]{Linked Open Data}
\acrodef{LODE}[LODE]{Linking Open Descriptions of Events}
\acrodef{LpO}[LpO]{Leave-$p$-Out}
\acrodef{LRE}[LRE]{Local Rank Error}
\acrodef{LRM}[LRM]{Local Relational Model}
\acrodef{LRU}[LRU]{Last Recently Used}
\acrodef{LS}[LS]{Lexical Signature}
\acrodef{LSM}[LSM]{Log Storing Manager}
\acrodef{LtR}[LtR]{Learning to Rank}
\acrodef{LUG}[LUG]{Lexical Unit Generator}
\acrodef{MA}[MA]{Mobile Agent}
\acrodef{MA}[MA]{Moving Average}
\acrodef{MACS}[MACS]{Multilingual ACcess to Subjects}
\acrodef{MADCOW}[MADCOW]{Multimedia Annotation of Digital Content Over the Web}
\acrodef{MAD}[MAD]{Mean Assessed Documents}
\acrodef{MADP}[MADP]{Mean Assessed Documents Precision}
\acrodef{MADS}[MADS]{Metadata Authority Description Standard}
\acrodef{MAP}[MAP]{Mean Average Precision}
\acrodef{MARC}[MARC]{Machine Readable Cataloging}
\acrodef{MATTERS}[MATTERS]{MATlab Toolkit for Evaluation of information Retrieval Systems}
\acrodef{MDA}[MDA]{Model Driven Architecture}
\acrodef{MDD}[MDD]{Model-Driven Development}
\acrodef{METS}[METS]{Metadata Encoding and Transmission Standard}
\acrodef{MIDI}[MIDI]{Musical Instrument Digital Interface}
\acrodef{MIME}[MIME]{Multipurpose Internet Mail Extensions}
\acrodef{ML}[ML]{Machine Learning}
\acrodef{MLIA}[MLIA]{MultiLingual Information Access}
\acrodef{MM}[MM]{Machinery Model}
\acrodef{MMU}[MMU]{Memory Management Unit}
\acrodef{MODS}[MODS]{Metadata Object Description Schema}
\acrodef{MOF}[MOF]{Meta-Object Facility}
\acrodef{MP}[MP]{Markov Precision}
\acrodef{MPEG}[MPEG]{Motion Picture Experts Group}
\acrodef{MRD}[MRD]{Machine Readable Dictionary}
\acrodef{MRF}[MRF]{Markov Random Field}
\acrodef{MS}[MS]{Mean Squares}
\acrodef{MSAC}[MSAC]{Multilingual Subject Access to Catalogues}
\acrodef{MSE}[MSE]{Mean Square Error}
\acrodef{MT}[MT]{Machine Translation}
\acrodef{MV}[MV]{Majority Vote}
\acrodef{MVC}[MVC]{Model-View-Controller}
\acrodef{NACSIS}[NACSIS]{NAtional Center for Science Information Systems}
\acrodef{NAP}[NAP]{Network processors Applications Profile}
\acrodef{NCP}[NCP]{Normalized Cumulative Precision}
\acrodef{nCG}[nCG]{Normalized Cumulated Gain}
\acrodef{nCRP}[nCRP]{Normalized Cumulated Relative Position}
\acrodef{nDCG}[nDCG]{Normalized Discounted Cumulated Gain}
\acrodef{nDE}[nDE]{Normalized Discounted Error}
\acrodef{NESTOR}[NESTOR]{NEsted SeTs for Object hieRarchies}
\acrodef{NEXI}[NEXI]{Narrowed Extended XPath I}
\acrodef{NII}[NII]{National Institute of Informatics}
\acrodef{NISO}[NISO]{National Information Standards Organization}
\acrodef{NIST}[NIST]{National Institute of Standards and Technology}
\acrodef{NLP}[NLP]{Natural Language Processing}
\acrodef{NLRE}[NLRE]{Normalized Local Rank Error}
\acrodef{NN}[NN]{Neural Network}
\acrodef{NP}[NP]{Network Processor}
\acrodef{NR}[NR]{Normalized Recall}
\acrodef{NS-M}[NS-M]{Nested Set Model}
\acrodef{NTCIR}[NTCIR]{NII Testbeds and Community for Information access Research}
\acrodef{OAI}[OAI]{Open Archives Initiative}
\acrodef{OAI-ORE}[OAI-ORE]{Open Archives Initiative Object Reuse and Exchange}
\acrodef{OAI-PMH}[OAI-PMH]{Open Archives Initiative Protocol for Metadata Harvesting}
\acrodef{OAIS}[OAIS]{Open Archival Information System}
\acrodef{OC}[OC]{Operation Code}
\acrodef{OCLC}[OCLC]{Online Computer Library Center}
\acrodef{OMG}[OMG]{Object Management Group}
\acrodef{OO}[OO]{Object Oriented}
\acrodef{OODB}[OODB]{Object-Oriented \acs{DB}}
\acrodef{OODBMS}[OODBMS]{Object-Oriented \acs{DBMS}}
\acrodef{OPAC}[OPAC]{Online Public Access Catalog}
\acrodef{OQL}[OQL]{Object Query Language}
\acrodef{ORP}[ORP]{Open Relevance Project}
\acrodef{OSIRIS}[OSIRIS]{Open Service Infrastructure for Reliable and Integrated process Support}
\acrodef{P}[P]{Precision}
\acrodef{P2P}[P2P]{Peer-To-Peer}
\acrodef{PA}[PA]{Performance Analysis}
\acrodef{PAMT}[PAMT]{Pool-Assessment Management Tool}
\acrodef{PASM}[PASM]{Pool-Assessment Storing Manager}
\acrodef{PC}[PC]{Program Counter}
\acrodef{PCP}[PCP]{Pre-Commercial Procurement}
\acrodef{PCR}[PCR]{Peripherical Command Register}
\acrodef{PDA}[PDA]{Personal Digital Assistant}
\acrodef{PDF}[PDF]{Probability Density Function}
\acrodef{PDR}[PDR]{Peripherical Data Register}
\acrodef{PIR}[PIR]{Personalized Information Retrieval}
\acrodef{POI}[POI]{\acs{PURL}-based Object Identifier}
\acrodef{PoS}[PoS]{Part of Speech}
\acrodef{PPE}[PPE]{Programmable Processing Engine}
\acrodef{PREFORMA}[PREFORMA]{PREservation FORMAts for culture information/e-archives}
\acrodef{PRIMAmob-UML}[PRIMAmob-UML]{mobile \acs{PRIMA-UML}}
\acrodef{PRIMA-UML}[PRIMA-UML]{PeRformance IncreMental vAlidation in \acs{UML}}
\acrodef{PROM}[PROM]{Programmable \acs{ROM}}
\acrodef{PROMISE}[PROMISE]{Participative Research labOratory  for Multimedia and Multilingual Information Systems Evaluation}
\acrodef{pSQL}[pSQL]{propagate \acs{SQL}}
\acrodef{PUI}[PUI]{Participant User Interface}
\acrodef{PURL}[PURL]{Persistent \acs{URL}}
\acrodef{QA}[QA]{Question Answering}
\acrodef{QoS-UML}[QoS-UML]{\acs{UML} Profile for QoS and Fault Tolerance}
\acrodef{QPA}[QPA]{Query Performance Analyzer}
\acrodef{R}[R]{Recall}
\acrodef{RAM}[RAM]{Random Access Memory}
\acrodef{RAMM}[RAM]{Random Access Machine}
\acrodef{RBO}[RBO]{Rank-Biased Overlap}
\acrodef{RBP}[RBP]{Rank-Biased Precision}
\acrodef{RDBMS}[RDBMS]{Relational \acs{DBMS}}
\acrodef{RDF}[RDF]{Resource Description Framework}
\acrodef{REST}[REST]{REpresentational State Transfer}
\acrodef{REV}[REV]{Remote Evaluation}
\acrodef{RFC}[RFC]{Request for Comments}
\acrodef{RIA}[RIA]{Reliable Information Access}
\acrodef{RMSE}[RMSE]{Root Mean Square Error}
\acrodef{RMT}[RMT]{Run Management Tool}
\acrodef{ROM}[ROM]{Read Only Memory}
\acrodef{ROMIP}[ROMIP]{Russian Information Retrieval Evaluation Seminar}
\acrodef{RoMP}[RoMP]{Rankings of Measure Pairs}
\acrodef{RoS}[RoS]{Rankings of Systems}
\acrodef{RP}[RP]{Relative Position}
\acrodef{RR}[RR]{Reciprocal Rank}
\acrodef{RSM}[RSM]{Run Storing Manager}
\acrodef{RST}[RST]{Rhetorical Structure Theory}
\acrodef{RT-UML}[RT-UML]{\acs{UML} Profile for Schedulability, Performance and Time}
\acrodef{SA}[SA]{Software Architecture}
\acrodef{SAL}[SAL]{Storing Abstraction Layer}
\acrodef{SAMT}[SAMT]{Statistical Analysis Management Tool}
\acrodef{SAN}[SAN]{Sistema Archivistico Nazionale}
\acrodef{SASM}[SASM]{Statistical Analysis Storing Manager}
\acrodef{SD}[SD]{Sequence Diagram}
\acrodef{SE}[SE]{Search Engine}
\acrodef{SEBD}[SEBD]{Convegno Nazionale su Sistemi Evoluti per Basi di Dati}
\acrodef{SERP}[SERP]{Search Engine Result Page}
\acrodef{SFT}[SFT]{Satisfaction--Frustration--Total}
\acrodef{SIL}[SIL]{Service Integration Layer}
\acrodef{SIP}[SIP]{Submission Information Package}
\acrodef{SKOS}[SKOS]{Simple Knowledge Organization System}
\acrodef{SM}[SM]{Software Model}
\acrodef{SME}[SME]{Statistics--Metrics-Experiments}
\acrodef{SMART}[SMART]{System for the Mechanical Analysis and Retrieval of Text}
\acrodef{SoA}[SoA]{Service-oriented Architectures}
\acrodef{SOA}[SOA]{Strength of Association}
\acrodef{SOAP}[SOAP]{Simple Object Access Protocol}
\acrodef{SOM}[SOM]{Self-Organizing Map}
\acrodef{SPARQL}[SPARQL]{Simple Protocol and RDF Query Language}
\acrodef{SPE}[SPE]{Software Performance Engineering}
\acrodef{SPINA}[SPINA]{Superimposed Peer Infrastructure for iNformation Access}
\acrodef{SPLIT}[SPLIT]{Stemming Program for Language Independent Tasks}
\acrodef{SPOOL}[SPOOL]{Simultaneous Peripheral Operations On Line}
\acrodef{SQL}[SQL]{Structured Query Language}
\acrodef{SR}[SR]{Sliding Ratio}
\acrodef{SR}[SR]{Status Register}
\acrodef{SRU}[SRU]{Search/Retrieve via \acs{URL}}
\acrodef{SS}[SS]{Sum of Squares}
\acrodef{SSTF}[SSTF]{Shortest Seek Time First}
\acrodef{STAR}[STAR]{Steiner-Tree Approximation in Relationship graphs}
\acrodef{STON}[STON]{STemming ON}
\acrodef{SVM}[SVM]{Support Vector Machine}
\acrodef{TAC}[TAC]{Text Analysis Conference}
\acrodef{TBG}[TBG]{Time-Biased Gain}
\acrodef{TCP}[TCP]{Transmission Control Protocol}
\acrodef{TEL}[TEL]{The European Library}
\acrodef{TERRIER}[TERRIER]{TERabyte RetrIEveR}
\acrodef{TF}[TF]{Term Frequency}
\acrodef{TFR}[TFR]{True False Rate}
\acrodef{TLD}[TLD]{Top Level Domain}
\acrodef{TME}[TME]{Topics--Metrics-Experiments}
\acrodef{TN}[TN]{True Negative}
\acrodef{TO}[TO]{Transfer Object}
\acrodef{TP}[TP]{True Positve}
\acrodef{TPR}[TPR]{True Positive Rate}
\acrodef{TRAT}[TRAT]{Text Relevance Assessing Task}
\acrodef{TREC}[TREC]{Text REtrieval Conference}
\acrodef{TRECVID}[TRECVID]{TREC Video Retrieval Evaluation}
\acrodef{TTL}[TTL]{Time-To-Live}
\acrodef{UCD}[UCD]{Use Case Diagram}
\acrodef{UDC}[UDC]{Universal Decimal Classification}
\acrodef{uGAP}[uGAP]{User-oriented Graded Average Precision}
\acrodef{UI}[UI]{User Interface}
\acrodef{UML}[UML]{Unified Modeling Language}
\acrodef{UMT}[UMT]{User Management Tool}
\acrodef{UMTS}[UMTS]{Universal Mobile Telecommunication System}
\acrodef{UoM}[UoM]{Utility-oriented Measurement}
\acrodef{UPC}[UPC]{Universal Product Code}
\acrodef{URI}[URI]{Uniform Resource Identifier}
\acrodef{URL}[URL]{Uniform Resource Locator}
\acrodef{URN}[URN]{Uniform Resource Name}
\acrodef{USM}[USM]{User Storing Manager}
\acrodef{VA}[VA]{Visual Analytics}
\acrodef{VAIRE}[VAIR\"{E}]{Visual Analytics for Information Retrieval Evaluation}
\acrodef{VATE}[VATE$^2$]{Visual Analytics Tool for Experimental Evaluation}
\acrodef{VIRTUE}[VIRTUE]{Visual Information Retrieval Tool for Upfront Evaluation}
\acrodef{VD}[VD]{Virtual Document}
\acrodef{VDM}[VDM]{Visual Data Mining}
\acrodef{VIAF}[VIAF]{Virtual International Authority File}
\acrodef{VL}[VL]{Visual Language}
\acrodef{VoIP}[VoIP]{Voice over IP}
\acrodef{VS}[VS]{Visual Sentence}
\acrodef{W3C}[W3C]{World Wide Web Consortium}
\acrodef{WAN}[WAN]{Wide Area Network}
\acrodef{WHO}[WHO]{World Health Organization}
\acrodef{WLAN}[WLAN]{Wireless \acs{LAN}}
\acrodef{WP}[WP]{Work Package}
\acrodef{WS}[WS]{Web Services}
\acrodef{WSD}[WSD]{Word Sense Disambiguation}
\acrodef{WSDL}[WSDL]{Web Services Description Language}
\acrodef{WWW}[WWW]{World Wide Web}
\acrodef{XMI}[XMI]{\acs{XML} Metadata Interchange}
\acrodef{XML}[XML]{eXtensible Markup Language}
\acrodef{XPath}[XPath]{XML Path Language}
\acrodef{XSL}[XSL]{eXtensible Stylesheet Language}
\acrodef{XSL-FO}[XSL-FO]{\acs{XSL} Formatting Objects}
\acrodef{XSLT}[XSLT]{\acs{XSL} Transformations}
\acrodef{YAGO}[YAGO]{Yet Another Great Ontology}
\acrodef{YASS}[YASS]{Yet Another Suffix Stripper}


==> sections/analysis.tex <==
\section{Task and Dataset}
\label{sec:analysis}

%\subsection{Task Description}

The TREC-COVID Challenge was a standard AdHoc task with the purpose of developing and evaluate IR systems able to assists scientists, clinicians, policy makers, and others to manage the rapidly growing corpus of scientific literature related to COVID-19. Participants were provided with a corpus of documents and a set of topics, and they had to return a list of $1\,000$ documents for each topic, where the documents at the beginning of the list are supposed to be the most relevant with respect to the topic.

The challenge was organized in several subsequent rounds, $5$ in total. At the beginning of each round a new portion of the corpus was released together with a set of topics. At the end of each round NIST was collecting the submitted runs and creating the pool of documents to be assessed. Assessors were biomedical experts from NLM, OHSU, and UTHealth. Topics, runs, relevance assessments and evaluation results are publicly availabe online\footnote{\url{https://ir.nist.gov/covidSubmit/archive.html}}.

In the following we provide a brief description of the corpus (Section~\ref{subsec:corpus}), the topics (Section~\ref{subsec:topics}), the relevance assessments (Section~\ref{subsec:rel_assessments}), and some statistics we conducted after Round $1$ assessments were released (section~\ref{subsec:stat}). More details can be found in the challenge overview~\cite{roberts2020trec,voorhees2020trec}.

\subsection{Corpus}
\label{subsec:corpus}

The corpus used throughout the challenge was the CORD-19: COVID-19 Open Research Dataset~\cite{Wang2020CORD19TC}\footnote{\url{https://www.semanticscholar.org/cord19}}.
The dataset contains research papers on COVID-19 and coronaviruses collected from PubMed, WHO, bioRxiv and medRxiv. 
The dataset is updated regularly, as new research papers are published, therefore, each round of the challenge exploited a specific release of the CORD-19 dataset\footnote{\url{https://ir.nist.gov/covidSubmit/data.html}}.

In addition to the documents, the dataset contains a metadata file. 
The list of metadata with their description is reported in Table~\ref{tab:metadata}.

\begin{table}[htb]
\caption{Metadata, description and statistics form CORD-19 version \td{@Lucas: Please add the version of CORD-19 dataset used to get this data.}.}
\label{tab:metadata}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}llc@{}}
\toprule
Metadata & Description & Number of instances \\ \midrule
cord\_uid & Each unique paper object receives a corresponding `cord\_uid'. & 51078 \\
title & Title of the article & 50920 \\
doi & Digital object identifier & 47741 \\
url & Source url of the article & 50776 \\
pmcid & PubMed Central (PMC) identifier & 41082 \\
pubmed\_id & Pubmed Identifier & 37861 \\
abstract & Full abstract & 42352 \\
has\_full\_text & Gives the name of the subset file that includes the full text of this paper. & 38022 \\
publish\_time & Time of publication & 19167 \\
authors & Author list of the article & 48891 \\
Microsoft Academic Paper ID & Microsoft Academic ID mapping & 964 \\
WHO \#Covidence & World Health Organization (WHO) Covidence Identifier & 1768 \\ \bottomrule
\end{tabular}%
}
\end{table}

\subsection{Topics}
\label{subsec:topics}

A total of $50$ topics were released throughout the entire challenge: $30$ topics were initially released at round $1$, and then $5$ extra topics were released for each following round. Topics were created by biomedical experts, who took inspiration from questions submitted to the National Library of Medicine (NLM) search service and discussions on social media.

An example of topic is shown in Figure~\ref{fig:topic}.
Each topic has $3$ fields: a title, which provides keywords to represent the information need; a question, to better specify the information need; and a narrative which provides extra clarifications.

\begin{figure}[htb]
\begin{Verbatim}
<topic number="1">
<query>coronavirus origin</query>
<question>what is the origin of COVID-19</question>
<narrative>seeking range of information about the SARS-CoV-2 virus's origin, including 
its evolution, animal source, and first transmission into humans</narrative>
</topic>
\end{Verbatim}
\caption{Example of topic for the TREC COVIDSearch 2020.}
\label{fig:topic}
\end{figure}

\subsection{Relevance Assessments}
\label{subsec:rel_assessments}

%pool

Relevance assessments were collected at the end of each round. 
The assessors used a $3$-grade scale: ``Relevant'', if the document provides an answer to the topic question substantiated by the necessary information, ``Partially Relevant'', if the document does not provide a complete answer to the topic question and further information is needed, or ``Not Relevant'', in all other cases.

For each round, the submitted runs were evaluated with NDCG@K, Precision@K, Brepf, RBP ($p=0.5$), and MAP, with a varying cut-off $K$. 
All measures were computed with \texttt{trec\_eval}\footnote{\url{https://github.com/usnistgov/trec_eval}}.

%\subsection{Analysis of Metadata}

% \begin{table}[htb]
% \caption{Metadata description and statistics.}
% \label{tab:metadata}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}lll@{}}
% \toprule
% \textbf{Metadata} & \textbf{Description} & \textbf{Number of instances} \\ \midrule
% cord\_uid & Each unique paper object receives a corresponding `cord\_uid'. & 45,774 \\
% title & Title of the article & 45,617 \\
% doi & Digital object identifier & 42,440 \\
% url & Source url of the article & 45,472 \\
% pmcid & PubMed Central (PMC) identifier & 26,243 \\
% pubmed\_id & Pubmed Identifier & 34,641 \\
% abstract & Full abstract & 37,913 \\
% has\_full\_text & Gives the name of the subset file that includes the full text of this paper. & 31,753 \\
% publish\_time & Time of publication & 45,765 \\
% authors & Author list of the article & 43,774 \\
% sha & \begin{tabular}[c]{@{}l@{}}Gives the associated filenames in the subset file \\ (some rows have multiple entries in the `sha' column, separated by `;'\\ with some additional files)\end{tabular} & {[}`nan': 14021, `1':29,206, `2+':1547{]} \\
% %sha & & {[}`nan': 14021, `1':29,206, `2+':1547{]} \\
% source\_x & Metadata for papers from these sources are combined: WHO, CZI, PMC, BioRxiv/MedRxiv, Elsevier & \begin{tabular}[c]{@{}l@{}}\{'biorxiv': 631, 'medrxiv': 587,'CZI': 164, \\ 'WHO': 1102, 'PMC': 24595, 'Elsevier': 18695\}\end{tabular} \\
% license & Corresponds to the publication license of the paper (each folder of the dataset) & \begin{tabular}[c]{@{}l@{}}\{'biorxiv': 631,'medrvix': 587,'cc-by-nc-nd': 668,\\          'cc-by': 8858,'cc-by-nc': 1160,'cc-by-nc-sa': 472,\\          'pd': 3,'unk': 10803,'no-cc': 3631,'cc0': 260,'cc-by-sa': 2,\\          'cc-by-nd': 4,'els-covid': 18695\}\end{tabular} \\
% journal & Journal & \begin{tabular}[c]{@{}l@{}}41707 - Most Common: {[}('Journal of Virology', 1740),  ('PLoS One', 1567),\\  ('Virology', 865), ('Emerg Infect Dis', 749){]}\end{tabular} \\
% Microsoft Academic Paper ID & Microsoft Academic ID mapping & 964 \\
% WHO \#Covidence & World Health Organization (WHO) Covidence Identifier & 1768 \\
% full\_text\_file & Gives the name of the subset file that includes the full text of this paper (also available in license column) & \begin{tabular}[c]{@{}l@{}}\{'biorxiv\_medrxiv': 1218, noncomm\_use\_subset': 2131,\\  'comm\_use\_subset': 8982, 'nan': 10216, 'custom\_license': 23227\}\end{tabular} \\
%  \bottomrule
% \end{tabular}%
% }
% \end{table}

% \begin{table}[h!]
% \caption{Metadata description and statistics.}
% \label{tab:metadata}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}llc@{}}
% \toprule
% Metadata & Description & Number of instances \\ \midrule
% cord\_uid & Each unique paper object receives a corresponding `cord\_uid'. & 51078 \\
% title & Title of the article & 50920 \\
% doi & Digital object identifier & 47741 \\
% url & Source url of the article & 50776 \\
% pmcid & PubMed Central (PMC) identifier & 41082 \\
% pubmed\_id & Pubmed Identifier & 37861 \\
% abstract & Full abstract & 42352 \\
% has\_full\_text & Gives the name of the subset file that includes the full text of this paper. & 38022 \\
% publish\_time & Time of publication & 19167 \\
% authors & Author list of the article & 48891 \\
% Microsoft Academic Paper ID & Microsoft Academic ID mapping & 964 \\
% WHO \#Covidence & World Health Organization (WHO) Covidence Identifier & 1768 \\ \bottomrule
% \end{tabular}%
% }
% \end{table}

% \begin{itemize}
%     \item Not every document has full text.
%     \item Some articles do not have a title, which is strange.
%     \item Some of them do not have a url (how was it crawled?)
%     \item Should we also index additional information from the ``sha" row in Table~\ref{tab:metadata}?
% \end{itemize}


\subsection{Analysis of Round 1 Qrels}
\label{subsec:stat}

\begin{table}[h!]
\caption{Analysis of relevance assessments for round 1. Number of judged documents for each relevance degree and overall statistics.}
\label{tab:qrels_round1_relevance}
\centering
\begin{tabular}{@{}lllll@{}}
\toprule
Topic ID              & Not Relevant ($0$) & Partially Relevant ($1$) & Relevant ($2$) & Sum \\ \midrule
1   & 222   & 45    & 56    & 323   \\
2   & 237   & 21    & 26    & 284   \\
3   & 247   & 66    & 24    & 337   \\
4   & 298   & 32    & 27    & 357   \\
5   & 205   & 35    & 96    & 336   \\
6   & 158   & 80    & 83    & 321   \\
7   & 226   & 247   & 7     & 275   \\
8   & 284   & 46    & 30    & 360   \\
9   & 257   & 25    & 16    & 298   \\
10  & 106   & 35    & 50    & 191   \\
11  & 272   & 67    & 5     & 344   \\
12  & 122   & 76    & 126   & 324   \\
13  & 227   & 97    & 49    & 373   \\
14  & 193   & 24    & 5     & 222   \\
15  & 291   & 45    & 12    & 348   \\
16  & 287   & 42    & 11    & 340   \\
17  & 166   & 32    & 45    & 243   \\
18  & 156   & 79    & 32    & 267   \\
19  & 258   & 27    & 16    & 301   \\
20  & 181   & 41    & 25    & 247   \\
21  & 234   & 15    & 70    & 319   \\
22  & 212   & 17    & 30    & 259   \\
23  & 230   & 4     & 22    & 256   \\
24  & 216   & 14    & 19    & 249   \\
25  & 237   & 9     & 62    & 308   \\
26  & 187   & 19    & 106   & 312   \\
27  & 226   & 30    & 44    & 300   \\
28  & 142   & 9     & 29    & 180   \\
29  & 118   & 42    & 58    & 218   \\
30  & 144   & 39    & 16    & 199   \\
\midrule
Sum & 6339  & 1115  & 1237  & 8691  \\
\midrule
\% of all assessments   & 72.9\%    & 12.8\%    & 14.2\%    &   \\
min & 106   & 2     & 5     & 180   \\
max & 298   & 97    & 126   & 373 \\
average & 211.3 & 37.2  & 41.2  & 289.7 \\
\midrule
\multicolumn{4}{l}{\hspace{-1em} Unique assessed docs = will be removed in round 2}   & 4778  \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[h!]
\caption{Count of the number of unique documents that were assessed as partially relevant ($1$) and/or relevant ($2$) over sources.}
\label{tab:qrels_round1_source}
\centering
\begin{tabular}{@{}lllll@{}}
\toprule
Source   & Partially Relevant ($1$) & Percentage & Relevant  ($2$) & Percentage \\ \midrule
arxiv    & $0$                      & $0\%$      & 1               & $0\%$      \\
biorxiv  & $45$                     & $5\%$      & 62              & $6\%$      \\
CZI      & $14$                     & $1\%$      & 14              & $1\%$      \\
Elsevier & $368$                    & $38\%$     & 372             & $35\%$     \\
medrxiv  & $178$                    & $18\%$     & 348             & $33\%$     \\
PMC      & $322$                    & $33\%$     & 192             & $18\%$     \\
WHO      & $41$                     & $4\%$      & 65              & $6\%$      \\
\midrule
Total    & $968$                    & $100\%$    & 1054            & $100\%$    \\ 
\bottomrule
\end{tabular}
\end{table}

\begin{table}[htb]
\caption{Count of the number of unique documents that were assessed as partially relevant ($1$) and/or relevant ($2$) over publication year.}
\label{tab:qrels_round1_year}
\centering
\begin{tabular}{@{}lllll@{}}
\toprule
PublicationYear & Partially Relevant ($1$) & Percentage & Partially Relevant ($2$) & Percentage \\ \midrule
1972            &                          & (0\%)      & 1                        & (0\%)      \\
1977            & 1                        & (0\%)      &                          & (0\%)      \\
1983            &                          & (0\%)      & 1                        & (0\%)      \\
1984            & 1                        & (0\%)      &                          & (0\%)      \\
1985            & 1                        & (0\%)      &                          & (0\%)      \\
1986            &                          & (0\%)      & 1                        & (0\%)      \\
1989            &                          & (0\%)      & 1                        & (0\%)      \\
1990            &                          & (0\%)      & 1                        & (0\%)      \\
1991            &                          & (0\%)      & 1                        & (0\%)      \\
1992            & 1                        & (0\%)      &                          & (0\%)      \\
1993            & 2                        & (0\%)      &                          & (0\%)      \\
1994            & 1                        & (0\%)      & 1                        & (0\%)      \\
1995            &                          & (0\%)      & 1                        & (0\%)      \\
1996            & 1                        & (0\%)      &                          & (0\%)      \\
1999            & 1                        & (0\%)      &                          & (0\%)      \\
2000            & 1                        & (0\%)      &                          & (0\%)      \\
2001            & 1                        & (0\%)      &                          & (0\%)      \\
2002            & 1                        & (0\%)      &                          & (0\%)      \\
2003            & 10                       & (1\%)      & 4                        & (0\%)      \\
2004            & 28                       & (3\%)      & 26                       & (2\%)      \\
2005            & 24                       & (2\%)      & 21                       & (2\%)      \\
2006            & 19                       & (2\%)      & 24                       & (2\%)      \\
2007            & 6                        & (1\%)      & 13                       & (1\%)      \\
2008            & 20                       & (2\%)      & 15                       & (1\%)      \\
2009            & 19                       & (2\%)      & 6                        & (1\%)      \\
2010            & 23                       & (2\%)      & 8                        & (1\%)      \\
2011            & 20                       & (2\%)      & 11                       & (1\%)      \\
2012            & 12                       & (1\%)      & 5                        & (0\%)      \\
2013            & 17                       & (2\%)      & 10                       & (1\%)      \\
2014            & 19                       & (2\%)      & 12                       & (1\%)      \\
2015            & 24                       & (2\%)      & 12                       & (1\%)      \\
2016            & 40                       & (4\%)      & 10                       & (1\%)      \\
2017            & 33                       & (3\%)      & 11                       & (1\%)      \\
2018            & 38                       & (4\%)      & 9                        & (1\%)      \\
2019            & 40                       & (4\%)      & 16                       & (2\%)      \\
2020            & 563                      & (58\%)     & 832                      & (79\%)     \\
\midrule
                & 967                      & (100\%)    & 1053                     & (100\%)    \\ \bottomrule
\end{tabular}
\end{table}

Disagreement analysis between the official qrels from NIST and our relevance judgements:
\begin{itemize}
    \item Common labels, i.e.~documents that were assessed by us and NIST: $243$
    \item Documents assessed only by us: $55$
    \item Agreed labels: $127$ $(52.3\%)$
    \item Disagreed labels: $116$ $(47.7\%)$
    \item Id-errors mapping: $3$
\end{itemize}

\clearpage

==> sections/approach.tex <==
\section{Approach}
\label{sec:approach}


% \td{@Lucas: Please add details about the index, where does it come from (Anserini- Jimmy Lin), and the $3$ different types of indexes. Information about tokenization, stopwords, stemming, normalization and other preprocessing steps.}

\subsection{Round 1}

\paragraph{RunID: KU\_run1}
This is a baseline run using BM25 implementation from Indri Search engine with $k_1=1.2$ and $b=0.75$. After retrieving the initial ranking, we re-rank the top-50 documents prioritizing articles published in 2020.
 
\paragraph{RunID: KU\_run2}
This run implements query expansion using external data sources with different weights for different types of expanded terms. The external data sources we employ include Human Disease Ontology (HDO)\footnote{\url{https://www.ebi.ac.uk/ols/ontologies/doid}} and Lexigram API. 

The HDO has been developed as a standardized human disease ontology, playing the role of providing consistent, reusable, and sustainable descriptions of human disease terms. As HDO is organized hierarchically, we retrieve the parent-class and the sub-class disease concepts. For example, for the coronavirus (COVID-19) we found that the "COVID-19" is a leaf concept and its parent concept is "coronavirus infection" whose further parent concept is "viral infectious diseas".

From Lexigram, we extract the entities from the original queries and types of entities. As a result, a query is expanded with potentially alternative disease terms, entity labels, and entity types.

%Specifically, we assign original query terms with weight 1.0, alternative disease terms 0.7, entity labels 0.4, and entity types 0.1. In practice, we use the Indri Language Model with Dirichlet smoothing with mu=2500.

We weigh these expanded terms based on the weighting schema of~\citet{faesslerjulie}. Specifically, we assign the following weights: original query terms weight $1.0$; alternative disease terms $0.7$; entity labels $0.4$; and entity types $0.1$. In practice, we employ the Indri search engine, where we achieve our settings with the operator \texttt{\#weight}.


%\subsection{Query Expansion based retrieval}
%\dw{About the Query Expansion Submission}
%We expand the queries by taking advantages of external data sources; and empirically add different weights for different types of expanded terms. The external datasources we employ include Human Disease Ontology (HDO)\footnote{https://www.ebi.ac.uk/ols/ontologies/doid} and Lexigram API. The HDO has been developed as a standardized human disease ontology, playing the role of providing consistent, reusable and sustainable descriptions of human disease terms. 

%As HDO is organized in a hierarchical manner, we retrieve the parent-class and the sub-class disease concepts. For example, for the coronavirus (COVID-19) we investigate on, we found that the "COVID-19" is a leaf concept and its parent concept is "coronavirus infection" whose further parent concept is "viral infectious disease". For Lexigram, we use it to extract the entities from the original queries, then the types of the entities. As a result, a query is expanded with potentially alternative disease terms, entity labels, and entity types. 

% We weigh these expanded terms based on our empirical sense with reference to the weighting schema of \citet{faesslerjulie}. Specifically, we assign original query terms with weight 1.0, alternative disease terms 0.7, entity labels 0.4, and entity types 0.1. In practive, we employ indri search engine where we achieve our settings with the operator ’\#weight'.
 
\paragraph{RunID: KU\_run3}
First, we built a paragraph-level index where we create a document for indexing comprising the title, abstract, and that paragraph.
We use BM25 implementation from the Indri Search engine with $k_1=1.2$ and $b=0.75$ to generate an initial ranking. After retrieving the initial ranking, we re-rank the top-50 documents prioritizing articles published in 2020. Next, using the pre-trained BioBERT from the HuggingFace Transformer library we generate representations of each paragraph and queries, compute the similarity between both, and finally re-sort the documents according to each similarity score.




%\td{@Lucas: index the collection yourself with Indri, please also specify here the parameters that you used to index the collection.}


%\td{@Casper: work with word embeddings?} \lcl{I have found a sample code from Jimmy Lin that uses SciBert+pyserini. It is straightforward and it uses the library transformers.}

% \subsection{Round 2:}

% All the submitted runs are built on top of the following $3$ steps.\\
% \textbf{Step 0}: We create $3$ indexes: 
% \begin{enumerate}
%     \item Based on title and abstract;
%     \item Based on full-text;
%     \item Based on title, abstract and paragraph: each document is split into para1, para2, ..., paraK, and we create $K+1$ ``artificial'' documents of the form title+abstract, title+abstract+para1, title+abstract+para2.
% \end{enumerate}
% \textbf{Step 1}: We create $4$ different types of queries:
% \begin{enumerate}
% \item Query and named\_entitities(question);
% \item Query, named\_entitities(question) and named\_entitities(narrative);
% \item Question and named\_entitities(query);
% \item Question, named\_entitities(query) and named\_entitities(narrative).
% \end{enumerate}
% \textbf{Step 2}: For each query type we create $4$ runs (default BM25 + default RM3):
% \begin{enumerate}
%     \item We search in index of title and abstract;
%     \item We search in index of full-text;
%     \item We search in index of title, abstract and paragraph (where we only keep the first occurrence of a document and delete the following duplicates);
%     \item We search in index of title, abstract and paragraph (where we do not remove the duplicates).
% \end{enumerate}
% Exploiting these $4$ runs, we use reciprocal rank fusion to get $1$ run.

% By combining Step 1 and Step 2, we have $4$ fusion runs, which we use to create a final reciprocal rank fusion (Fusion of Fusions). We also create a fusion of the $16$ runs from Step 1 and Step 2, without an intermediate fusion (Fusion of Runs).

% \paragraph{RunID: fusionOfFusions} 

% We submitted the Fusion of Fusions run, i.e.~the run obtained by fusing the $4$ fused runs resulting from Step $1$ and Step $2$.

% \paragraph{RunID: allFiltering} 

% We use reciprocal rank fusion between the $27$ automatic runs, that did not contribute to the pooling, from round $1$, as well as our own $2$ fusion runs: Fusion of Fusions and Fusion of Runs. 

% \paragraph{RunID: soboroffFiltering}

% We use reciprocal rank fusion between the $9$ automatic runs, that did not contribute to the pooling and was chosen based on the middle runs from Soboroff's Method~\citep{SoboroffEtAl2001,SakaietAl2010} out of $27$ possible runs, from round $1$, as well as our own $2$ fusion runs: Fusion of Fusions and Fusion of Runs.


% \vspace{2em}
% For more details on Casper's runs: \url{https://docs.google.com/document/d/1CL5JT5HthYlnuweH3VC2I8dF8fDopJGObLqPfzzWyQA/edit?usp=sharing}

\subsection{Round 2 and 3}
In round 2 and 3 we explored fusion-based approaches based on creating multiple query variations per topic, which are used for searching within different types of indexes. Specifically, we first create three indexes:
\begin{itemize}
    \item We build an index based on the title and abstract of each document;
    \item We build an index based on the full text of each document;
    \item Each document is split into its paragraphs, such that from each paragraph a new \emph{artificial} document is constructed based on the title, abstract, and paragraph. We build an index based on these constructed paragraph-level documents.
\end{itemize}
For constructing multiple queries per topic we use named entity recognition\footnote{\url{https://spacy.io/usage/linguistic-features\#named-entities}} 
to extract additional query terms based on different topic fields. We denote NE$(\cdot)$ as a function that extracts the named entities of a provided input text, and create four different query variations by combining the terms listed below:
\begin{itemize}
    \item Query and NE(question);
    \item Query, NE(question), and NE(narrative);
    \item Question and NE(query);
    \item Question, NE(query), and NE(narrative).
\end{itemize}
For each query variation we create 4 runs using BM25 with RM3 with default parameters\footnote{\url{https://github.com/castorini/pyserini}}:
\begin{itemize}
    \item We query the index of title and abstract;
    \item We query the index of full text;
    \item We query the paragraph-level index;
    \item We query the paragraph-level index, where we only keep the first occurrence of the original document id associated with each paragraph.
\end{itemize}
Based on these four runs, we apply Reciprocal Rank Fusion (RRF) \cite{cormack2009reciprocal} (using default $k=60$) to combine the four runs into one fused run. Finally, we submitted the following runs for round 2 and 3:
\begin{description}
    \item[Round 2 and 3 - RunID: fusionOfFusions] We obtain one fused run from each of the query variations (4 in total), which we further combine using RRF into a final run denoted as fusion of fusions.
    \item[Round 3 - RunID: fusionOfRuns] We obtain four runs for each of the query variations (16 in total), which we combine using RRF into a final run denoted as fusion of runs.
    
    \item[Round 2 - RunID: allFiltering] We apply RRF on all the automatic runs (27 in total), that did not contribute to the pooling from round 1, combined with our fusionOfFusions and fusionOfRuns runs. 
    \item[Round 2 - RunID: soboroffFiltering] We apply RRF on the 9 automatic runs, that did not contribute to the pooling and were chosen based on the 9 middle runs returned by applying Soboroff's method~\citep{SoboroffEtAl2001,SakaietAl2010} on the 27 runs that did not contribute to the pooling from round 1. Additionally, we include our fusionOfFusions and fusionOfRuns runs.
\end{description}

==> sections/conclusion.tex <==
\section{Discussion and Conclusion}
\label{sec:conclusion}

==> sections/experiments.tex <==
\section{Experimental Results and Analysis}
\label{sec:experiments}

\subsection{Round 1}
\label{subsec:round_1}
Draft explanation round1:
\begin{itemize}
    \item add bm25 alone to compare to our run with re-ranking and scibert.
    \item the re-ranking approach using the year is effective. The main reason why this approach work is because most of the documents that are considered relevant in Table(sortedbyyear) are more recent (2019+)
    \item Explain how our runs compare to the median of all the other runs.
    \item Our query expansion approach did not work well. One of the reasons can be due to the fact that by using the qery expansion approach in this covid-19 specific topic can lead to topic drift away from the specific topic. In addition, we did not re-rank by the year, and there are a lot of articles about corona virus related to animal, and query expansion can lead results towards that direction.
    \item Our run3 has imilar performance to the run1 without re-ranking using scibert. It is known that the contextual embedding tends to work better when fine-tuned to the specific task. One of the reasons can be due to the fact that we did not fine-tune the bert to this specific task. In this run we only used the pre-trained embedding and id not do any fine tunning to the retrieval task. 
    \item Compared to the best submitted run to the task, our approach perfom worse. However, we are still above the median for the task. 
\end{itemize}

\begin{table}[htb]
\centering
\caption{Official evaluation results for the runs submitted at round 1}
\label{tab:results_official_round1}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}llccccccccccc@{}}
\toprule
\textbf{run\_id} & \textbf{Description} & \multicolumn{1}{l}{\textbf{P@5}} & \multicolumn{1}{l}{\textbf{P@10}} & \multicolumn{1}{l}{\textbf{P@15}} & \multicolumn{1}{l}{\textbf{P@20}} & \multicolumn{1}{l}{\textbf{P@30}} & \multicolumn{1}{l}{\textbf{RPrec}} & \multicolumn{1}{l}{\textbf{NDCG@10}} & \multicolumn{1}{l}{\textbf{Bpref}} & \multicolumn{1}{l}{\textbf{MAP}} & \multicolumn{1}{l}{\textbf{\#relevant}} & \multicolumn{1}{l}{\textbf{\#rel ret}} \\ \midrule
KU\_run1 & BM25 + reranking by year & 0.5933 & 0.5367 & 0.5000 & 0.4567 & 0.3978 & 0.2559 & 0.4693 & 0.3814 & 0.2205 & 2352 & 1355 \\
KU\_run2 & \begin{tabular}[c]{@{}l@{}}Query expansion HDO \\ and LexicogramAPI\end{tabular} & 0.2600 & 0.2767 & 0.2711 & 0.2600 & 0.2356 & 0.1661 & 0.2308 & 0.3101 & 0.1010 & 2352 & 994 \\
KU\_run3 & \begin{tabular}[c]{@{}l@{}}BM25 + reranking with BERT\\ + reranking by year\end{tabular} & 0.5667 & 0.5567 & 0.5067 & 0.4667 & 0.3867 & 0.2555 & 0.4670 & 0.3787 & 0.2116 & 2352 & 1346 \\
\hdashline
sab20.1.meta.docs & \begin{tabular}[c]{@{}l@{}}SMART vector run,\\ Lnu docs and ltu queries.\end{tabular}  & 0.7800 & 0.7000 & 0.6333 & 0.5917 & 0.5211 & 0.3548 & 0.6080 & 0.4832 & 0.3128 & 2352 & 1778 \\ \bottomrule
\end{tabular}%
}
\end{table}



\begin{figure}[htbp]
\centering
\begin{subfigure}{.49\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/map.pdf}
  \caption{MAP scores}
  \label{fig:binary_useful}
\end{subfigure}
\begin{subfigure}{.49\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/ndcg10.pdf}
  \caption{NDCG@10 scores.}
  \label{fig:binary_useful_credible}
\end{subfigure}
\begin{subfigure}{.49\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/p10.pdf}
  \caption{Precision @10 scores.}
  \label{fig:binary_useful_correct}
\end{subfigure}
\begin{subfigure}{.49\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/num_rel_ret.pdf}
  \caption{Number of relevant documents retrieved.}
  \label{fig:binary_useful_correct_credible}
\end{subfigure}
\caption{Results of all submitted runs using map, nDCG@10, P@10 and number of relevant documents retrieved.}
\label{fig:binary_evaluation}
\end{figure}




\subsection{Round 2}

\begin{table}[htb]
\caption{Evaluation results on runs to be submitted on round 2. The results are with qrels for round 1 and corpus from round 1. }
\label{tab:results_round2_unofficial}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}llllll@{}}
\toprule
Run ID  & Name  & p@5   & ndcg@10 & map   & \#retrieved\_relevant \\
\midrule
 & Best automatic round 1: sab20.1.meta.docs    & 0.780 & 0.608   & 0.313 & 1778    \\
 & Best unjudged automatic round 1: run2    & 0.686 & 0.603   & 0.260 & 1220    \\
 & Best manual round 1: run1    & 0.793 & 0.684   & 0.263 & ?   \\
\midrule
 & Fusion of runs   & 0.713 & 0.628   & 0.382 & 1883    \\
\rowcolor[HTML]{DAE8FC} 
X   & Fusion of Fusions & 0.733 & 0.642   & 0.382 & 1899    \\
\midrule
 & Fusion all automatic unjudged runs (27 runs) & 0.800 & 0.699   & 0.460 & 2072 \\
 & Fusion all automatic unjudged runs + Fusion of Runs  & 0.806 & 0.706   & 0.464 & 2075 \\
 & Fusion all automatic unjudged runs + Fusion of Fusions   & 0.806 & 0.707   & 0.463 & 2075 \\
\rowcolor[HTML]{DAE8FC} 
X   & Fusion all automatic unjudged runs + Fusion of Runs + Fusion of Fusions   & 0.820 & 0.710   & 0.465 & 2070  \\
\midrule
 & Fusion of top 5 automatic unjudged runs  & 0.806 & 0.706   & 0.316 & 1655 \\
 & Fusion of top 5 + Fusion of Runs & 0.859 & 0.733   & 0.354 & 1822 \\
 & Fusion of top 5 + Fusion of Fusions  & 0.859 & 0.734   & 0.357 & 1825 \\
\rowcolor[HTML]{FFFFC7} 
\begin{tabular}[c]{@{}l@{}}Maybe X, but this is not \\ ``Pure'' no-tuning due \\ to our choice of runs.\end{tabular} & Fusion of top 5 + Fusion of Runs + Fusion of Fusions    & 0.866 & 0.740   & 0.379 & 1872  \\
\midrule
 & Fusion of Middle runs from Soboroff (9 runs out of 27 total) & 0.873 & 0.725   & 0.414 & 1989 \\
\rowcolor[HTML]{DAE8FC} 
X   & Fusion of Middle runs from Soboroff +  Fusion of Runs + Fusion of Fusions & 0.867 & 0.718   & 0.433 & 2008  \\ 
\bottomrule
\end{tabular}
}%
\end{table}

\clearpage

==> sections/extra_material.tex <==
\section{Extra Material: To be Removed}

% \mm{Useful links: 
% \begin{itemize}
%     \item Task description: \url{https://dmice.ohsu.edu/hersh/COVIDSearch.html};
%     \item Corpus: \url{https://pages.semanticscholar.org/coronavirus-research};
%     \item Useful information from Bispebjerg og Frederiksberg Hospital: \url{http://covid19medicin.dk/} translated version: \url{https://docs.google.com/document/d/1m-mL8-fIrjfgVyStBfRlrs5-RjmWX7JxXpF9gqPT4Uk/edit?ts=5e84acb5}
%     \item Another literature review: \url{https://www.kaggle.com/covid-19-contributions};
%     \item FAQ from danish government: \url{https://www.sst.dk/da/corona-eng/FAQ}
%     \item Guidelines and submission page: \url{https://ir.nist.gov/covidSubmit/}
% \end{itemize}
% }

Useful links related to the competition:
\begin{itemize}
    \item \textbf{Task description}:
    \begin{itemize}
        \item Description and guidelines: \url{https://ir.nist.gov/covidSubmit/round2.html}
        \item Official submission page: \url{https://ir.nist.gov/covidSubmit/}
    \end{itemize}
    \item \textbf{Experimental collection}:
    \begin{itemize}
        \item Corpus: \url{https://pages.semanticscholar.org/coronavirus-research}
        \item Topics and qrels: \url{https://ir.nist.gov/covidSubmit/data.html}
    \end{itemize}
    \item \textbf{Official experimental results:}
    \begin{itemize}
        \item Round 1 leaderboard: \url{https://docs.google.com/spreadsheets/d/1NOu3ZVNar_amKwFzD4tGLz3ff2yRulL3Tbg_PzUSR_U/edit#gid=1068033221}
        \item Round 1 runs: \url{https://ir.nist.gov/covidSubmit/archive/archive-round1.html}
    \end{itemize}
    \item \textbf{Documents about COVID to use as external resources}:
    \begin{itemize}
        \item Document from Bispebjerg og Frederiksberg Hospital: \url{http://covid19medicin.dk/} translated version: \url{https://docs.google.com/document/d/1m-mL8-fIrjfgVyStBfRlrs5-RjmWX7JxXpF9gqPT4Uk/edit?ts=5e84acb5}
        \item FAQ from danish government: \url{https://www.sst.dk/da/corona-eng/FAQ}
        \item Another literature review: \url{https://www.kaggle.com/covid-19-contributions}
    \end{itemize}
    \item \textbf{External computational resources}:
    \begin{itemize}
        \item Jimmy Linn's github with baselines: \url{https://github.com/castorini/anserini/blob/master/docs/experiments-covid.md}
        \item Jimmy Linn's github with indexing instruction: \url{https://github.com/castorini/anserini/blob/master/docs/experiments-cord19.md}
        \item Query expansion form Udel: \url{https://github.com/castorini/anserini/blob/master/src/main/python/trec-covid/generate_query_udel.py}
        \item Trectools for evaluation with python: \url{https://github.com/joaopalotti/trectools}
        \item Collection of public APIs for embedding scientific papers: \url{https://github.com/allenai/paper-embedding-public-apis\#specter}
    \end{itemize}
    \item \textbf{Research papers}:
    \begin{itemize}
        \item Google strategy on COVIDSearch: \url{https://arxiv.org/pdf/2004.14503.pdf}
        \item RM3 paper: \url{http://www.abdelali.net/ref/Lavrenko01RelevanceModels.pdf} 
        \item Jimmy Linn's paper to apply BERT with anserini: \url{https://www.aclweb.org/anthology/D19-3004.pdf}
    \end{itemize}
    
\end{itemize}

==> sections/introduction.tex <==
\section{Introduction}
\label{sec:introduction}


This report describes our participation to the COVIDSearch TREC competition, organised by TREC and NIST in 2020. The aim of the competition was to find the best information retrieval strategy for the task of searching for specialised Covid-19 related information in the biggest, to its day, collection of scientific literature on corona viruses. More than XX research groups joined this competition in the second half of 2020.

In the remainder of this paper, we present the task of the competition and the dataset (Section XX), our approach (Section XX), the empirical performance of our approach and a related analysis of these findings (Section XX), and a brief overview of highly related prior work in this area (Section XX).



==> sections/related.tex <==
\section{Brief Overview of Highly Relevant Prior Work}
\label{sec:related}



\subsection{Medical retrieval}
The successful submission in TREC 2019@PM (Precision Medicine) conducted by \citet{faesslerjulie} had their approach built upon carefully designed weighted queries according to their experience. Essentially, they expanded the queries to boost the recall with various tools and sources, e.g., Lexigram API. Lexigram is based on the Systematic Nomenclature of Medicine - Clinical Terms (SNOMED CT), Mesh, and ICD (International Classification of Disease). More importantly, they explored the query clause weighting schema by manually experimenting on their internal standard golds. As a result, the queries are formulated as ElasticSearch JSON queries that are delivered to ElasticSearch.


\citet{faesslerjulie} explored the usefulness of Learning to rank (LETOR), which worsened the results. Specifically, they implemented the LambdaMART (a list-wise approach), consisting of LambdaRank and MART (Multiple Additive Regression Tree), to train the model and rerank the documents. The four main features they use are:
Binary features for the 500 words with highest TF-IDF from the gold standard
Matches of the topic with the document
BM25 scores of the topic matched with document fields
FastText document embeddings of the document
As a result, however, the LETOR runs reveal decreased evaluation scores similarly to the Biomedical abstract task. The internal 2019 reference standard led to worse results than the union of previous official annotations.



Successful 2018@PM submission \cite{oleynik2018hpi} demonstrated that query expansion associated with hand-crafted rules led to better values of IR metrics. They expanded the topics for disease and gene. For instance, they enriched the diseases with their preferred term, synonyms, and hypernyms with Lexigram API. Also, they enriched their gene with their description and synonyms with the National Center for Biotechnology Information (NCBI). They gave the highest weight to the original topic and lower weights to the other terms. They provided the weight by extension type but did not provide any reasons for their decision. 

Successful 2017@PM submission
\cite{zhang2018can} raised the question "Can Word Embedding Help Term Mismatch Problem?'' particularly for clinical retrieval task. They found that word embedding can significantly improve low ranked relevant documents, with term mismatch problem being largely resolved; while for highly ranked documents with less term mismatching problem, word emending’s improvement can also be replaced by a traditional language model.

Pasche et al. \cite{pasche2017customizing} introduced an approach where the main component is a large query generation module, with each generated query being deferentially weighted. The reason is that they assume relevant abstracts that did not mention all critical aspects of the complete query still can be of interest. In addition, they applied hierarchical query expansion, as well as other empirical strategies, including priories publication type, defines a list of keywords as keywords density, etc.

\subsection{Word Embedding Oriented Retrieval Enhancement}
Due to specific domain (medical), \citet{nguyen2017learning} investigated how to optimize the document representation by leveraging neural-based approaches to capture latent representations built upon both validated medical concepts specified in an external resource as well as the used words. They validated their resulting document representation on two medical search tasks, health search, and clinical search, by showing the effectiveness. 

Some studies \cite{liu2016constraining,ling2017integrating} employed external knowledge bases to assist the representation of word embedding. Liu et al. \citet{liu2016constraining} leveraged the existing knowledge (word relations) in the medical domain to constrain word embeddings with the principle that related words should have similar embeddings. The underlying reason is that embeddings trained in an unsupervised manner may fail to capture some of the semantic relations in a specific area (e.g., healthcare). The adapted constrained word embeddings are used to rerank documents, demonstrating improved effectiveness to unsupervised word embeddings. 

Slightly different, Ling et al. \citet{ling2017integrating} studied to construct a weighted graph from knowledge bases (KBs) to represent structured relationships among words/concepts. They proposed a GCBOW model and a GSkip-gram model, respectively by integrating such a graph into the original CBOW model and Skip-gram model via graph regularization. They showed encouraging improvements with the new models on four general domain standard datasets and improved performance for biomedical Information Retrieval (IR) task.


%\td{@Dongsheng: Search related work with word embeddings.}

%\lcl{This is interesting, collection of public APIs for embedding scientific papers: \url{https://github.com/allenai/paper-embedding-public-apis\#specter}}
